Inference for extreme spatial temperature events in a changing climate with application to Ireland

We investigate the changing nature of the frequency, magnitude and spatial extent of extreme temperatures in Ireland from 1931 to 2022. We develop an extreme value model that captures spatial and temporal non-stationarity in extreme daily maximum temperature data. We model the tails of the marginal variables using the generalised Pareto distribution and the spatial dependence of extreme events by a semi-parametric Brown-Resnick r-generalised Pareto process, with parameters of each model allowed to change over time. We use weather station observations for modelling extreme events since data from climate models (not conditioned on observational data) can over-smooth these events and have trends determined by the specific climate model configuration. However, climate models do provide valuable information about the detailed physiography over Ireland and the associated climate response. We propose novel methods which exploit the climate model data to overcome issues linked to the sparse and biased sampling of the observations. Our analysis identifies a temporal change in the marginal behaviour of extreme temperature events over the study domain, which is much larger than the change in mean temperature levels over this time window. We illustrate how these characteristics result in increased spatial coverage of the events that exceed critical temperatures.

==> latexmkrc <==
# HACK: this width seems to change with every compile, so
# latexmk runs latex too many times; ignore it
$hash_calc_ignore_pattern{'aux'} = 'statsocwidth';

# All the other default settings on Overleaf
# support for the glossaries package:
add_cus_dep('glo', 'gls', 0, 'makeglossaries');
add_cus_dep('acn', 'acr', 0, 'makeglossaries');
sub makeglossaries {
  system("makeglossaries \"$_[0]\"");
}

# support for the nomencl package:
add_cus_dep('nlo', 'nls', 0, 'makenlo2nls');
sub makenlo2nls {
  system("makeindex -s nomencl.ist -o \"$_[0].nls\" \"$_[0].nlo\"");
}

# from the documentation for V. 2.03 of asymptote:
sub asy {return system("asy \"$_[0]\"");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

# metapost rule from http://tex.stackexchange.com/questions/37134
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}
